LED: Latent Variable-based Estimation of Density

Modern generative models are roughly divided into two main categories: (1) models that can produce high-quality random samples, but cannot estimate the exact density of new data points and (2) those that provide exact density estimation, at the expense of sample quality and compactness of the latent space. In this work we propose LED, a new generative model closely related to GANs, that allows not only efficient sampling but also efficient density estimation. By maximizing log-likelihood on the output of the discriminator, we arrive at an alternative adversarial optimization objective that encourages generated data diversity. This formulation provides insights into the relationships between several popular generative models. Additionally, we construct a flow-based generator that can compute exact probabilities for generated samples, while allowing low-dimensional latent variables as input. Our experimental results, on various datasets, show that our density estimator produces accurate estimates, while retaining good quality in the generated samples.

==> sections/discussion.tex <==
\section{Discussion}
\label{sec:Discussion and futurework}
\qheading{Future work:}
% \textcolor{red}{Connections to other models can come here, although I would put a subsection in Method}.
As noted in \secref{LED:gen_obj}, the computational efficiency of the normalizing constant, represented by \eqationref{int_as_expectation}, depends heavily on the similarity between the generator density $P_G(y)$ and the critic density $P_\theta(x)$. Since the generator and the critic network are initialized randomly and independently, this cannot be expected. We hypothesize that this slows down training in the beginning. Luckily, this can be addressed using a Metropolis-Adjusted over damped Langevin dynamics \cite{grenander1994representations}. Furthermore, these processes can be operated in the latent space of the generator and benefit from the smaller dimensionality of it. This, however, is deemed out of scope for the current study and left for future work.

In \secref{LED:sec:dim_red}, we make the assumption that in a natural image given an immediate neighbor, the distribution of the current pixel value is normally distributed. Although this holds for image data, it might not be true in general. One can relax this assumption and still maintain our workflow if an explicit density model (\eg autoregressive) is trained. Moreover, for random sampling and density evaluation at test time, this model will never be evaluated and hence one can afford to use a computationally expensive model. This is also deemed beyond the scope of this paper and left to future work.

Works that base their methods on log-likelihood maximization, such as VAEs, normalizing flow models, diffusion models and us, assume that the data lives in a continuous space they are expressed. This often might not be the case, and the data may live on a lower dimensional manifold. In such a scenario, the hyper area of support of it is zero. Hence, if the true probability density function is in the original space is a multidimensional Dirac delta function. Such functions are not easily learnable using gradient descent-based methods. Addressing this issue is deemed also out of scope of this paper and left to future work.
